A graded dependent type system with a usage-aware semantics (extended version)

Graded Type Theory provides a mechanism to track and reason about resource usage in type systems. In this paper, we develop GraD, a novel version of such a graded dependent type system that includes functions, tensor products, additive sums, and a unit type. Since standard operational semantics is resource-agnostic, we develop a heap-based operational semantics and prove a soundness theorem that shows correct accounting of resource usage. Several useful properties, including the standard type soundness theorem, non-interference of irrelevant resources in computation and single pointer property for linear resources, can be derived from this theorem. We hope that our work will provide a base for integrating linearity, irrelevance and dependent types in practical programming languages like Haskell.

==> Makefile <==
## Makefile for paper

BIBFILES   = weirich.bib eades.bib qtt.bib
OTT_SOURCE = ../simple/qtt extra

OTTFILES  = $(foreach i, $(OTT_SOURCE), $(i).ott) 
OTTIFLAGS = $(foreach i, $(OTT_SOURCE), -i $(i).ott) 
RULESFILE = qtt-rules.tex

TOP=paper
PDFS=paper.pdf

all: $(TOP).pdf
paper: $(TOP).pdf

%.tex: $(RULESFILE) %.mng Makefile 
	ott $(OTTIFLAGS) \
                    -tex_wrap false \
                    -tex_show_meta false \
                    -tex_filter $*.mng $*.tex

$(RULESFILE): $(OTTFILES)
	ott $(OTTIFLAGS) -o $(RULESFILE) \
          -tex_wrap false \
          -tex_show_meta false

%.pdf : $(TOP).tex $(BIBFILES) abstract.tex 
	latexmk -bibtex -pdf $(TOP).tex

response : popl2021-response.md	
	pandoc -f markdown -t latex popl2021-response.md -o popl2021-response-input.tex
	latexmk -pdf popl2021-response.tex

final-response : popl2021-final-response.md	
	pandoc -f markdown -t latex popl2021-final-response.md -o popl2021-final-response-input.tex
	latexmk -bibtex -pdf popl2021-final-response.tex

arxiv : paper
	mkdir -p arxiv
	cp $(TOP).tex $(RULESFILE) $(BIBFILES) abstract.tex *.cls *.sty arxiv/
	cd arxiv && make

paperclean:
	rm -if *-rules.tex $(TOP).tex *.log ./*~ *.aux $(PDFS) *.bbl *.blg *.fdb_latexmk *.fls *.out *-input.tex *~
	cd arxiv && make clean

clean: paperclean

